Measuring Interest Group Positions on Legislation: An AI-Driven Analysis of Lobbying Reports

Special interest groups (SIGs) in the U.S. participate in a range of political activities, such as lobbying and making campaign donations, to influence policy decisions in the legislative and executive branches. The competing interests of these SIGs have profound implications for global issues such as international trade policies, immigration, climate change, and global health challenges. Despite the significance of understanding SIGs' policy positions, empirical challenges in observing them have often led researchers to rely on indirect measurements or focus on a select few SIGs that publicly support or oppose a limited range of legislation. This study introduces the first large-scale effort to directly measure and predict a wide range of bill positions-Support, Oppose, Engage (Amend and Monitor)- across all legislative bills introduced from the 111th to the 117th Congresses. We leverage an advanced AI framework, including large language models (LLMs) and graph neural networks (GNNs), to develop a scalable pipeline that automatically extracts these positions from lobbying activities, resulting in a dataset of 42k bills annotated with 279k bill positions of 12k SIGs. With this large-scale dataset, we reveal (i) a strong correlation between a bill's progression through legislative process stages and the positions taken by interest groups, (ii) a significant relationship between firm size and lobbying positions, (iii) notable distinctions in lobbying position distribution based on bill subject, and (iv) heterogeneity in the distribution of policy preferences across industries. We introduce a novel framework for examining lobbying strategies and offer opportunities to explore how interest groups shape the political landscape.

==> figure_latex/bill_interest_group_bill_position.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{figure/kdeplot_2d_bill_interest_group_score.pdf}
\caption{Distribution of bill positions based on the bill ideal point and the latent preference of interest groups. The x-axis represents the latent preferences of interest groups, while the y-axis corresponds to the latent scores of bills. The plot highlights how the distribution of bill positions varies depending on both the interest group and the bill.}
\label{fig:bill_position_distribution}
\end{figure}

\begin{figure}[!thbp]
\centering
\includegraphics[width=\linewidth]{figure/one_bill_industry_bill_position_hr2474-116.pdf}
\caption{Comparison of bill position distribution by industry at the bill level. The y-axis represents the industry of interest groups, and the order is based on the descending average of all interest groups within each industry.}
\label{fig:one_bill_industry_bill_position}
\end{figure}

==> figure_latex/industry.tex <==
\begin{figure}[t!]
\centering
% \includegraphics[width=\linewidth]{figure/boxplot_ideal_point_by_industry.pdf}
\includegraphics[width=\linewidth]{figure/boxplot_industry.pdf}
\caption{Interest score Distribution by Industry. It shows the distribution of interest scores across 1,508 interest groups in 45 industries. The x-axis represents the average industry scores, arranged in descending order. Industries at the top are aligned with conservative ideologies or economic activities, while those at the bottom are associated with progressive values and social services. 6 industries with conflicting interest groups are highlighted, with opposing groups marked in the same color, clearly illustrating their contrasting positions.}
\label{fig:interest_score_distribution_industry}
\end{figure}


==> figure_latex/industry_bill_position_relation.tex <==
\begin{figure*}[!t]
\centering
\begin{subfigure}
    \centering
    \includegraphics[width=.3\linewidth]{figure/Circos_Plot_for_Lobbying_Network_Industry_Support.png}
    % \caption{Support network}
    \label{fig:support}
    \includegraphics[width=.3\linewidth]{figure/Circos_Plot_for_Lobbying_Network_Industry_Oppose.png}
    % \caption{Oppose network}
    \label{fig:oppose}
    \includegraphics[width=.3\linewidth]{figure/Circos_Plot_for_Lobbying_Network_Industry_Others.png}
    % \caption{Other networks}
    \label{fig:others}
\end{subfigure}
\caption{Visualization of lobbying networks by industry: (a) support, (b) oppose, and (c) other connections.}
\label{fig:lobbying_networks}
\end{figure*}

==> section/dataset.tex <==
% As a result, using our pipeline with LLM and GNN, we obtain a total of 279,104 bill position data across 12,032 interest groups and 42,475 bills as illustrated in Table~\ref{tab:bill_position_dataset_size}.

% By comparing our dataset with the existing MapLight bill position dataset, we highlight its broader coverage and scalability. Furthermore, we explain the differences between our data and the widely used metric for representing interest group latent scores, provided by DIME.

\paragraph{Comparison of Data Coverage with the MapLight Dataset}
We compare the scale of our dataset with the coverage of the existing human-curated MapLight bill position dataset, which spans the 111th to 115th Congress. Although our dataset covers a broader range (111th–117th Congress), the comparison remains meaningful as it demonstrates the scalability of our approach.
MapLight contains a total of 194,479 instances; however, when mapping interest group–bill pairs from lobbying reports~\footnote{\todo{Mapping is performed by searching the interest group's name in a search engine and identifying the first matching URL as the same entity.}}, 25,382 pairs remain, covering only a subset of the entities involved. Through this process, 25,382 pairs remain, covering 2,195 interest groups and 5,780 bills.
13.1\% of the MapLight dataset corresponds to our bill position data, while ours remains 11 times larger in instances. It also covers over five times more interest groups (12,032) and seven times more bills (42,475). The proposed pipeline provides a scalable framework that can be directly applied to future congressional data, minimizing the need for human annotation while significantly enhancing data coverage.

\paragraph{Interest Group Latent Preferences}
Similar to how roll call vote records are used to estimate politicians' ideal points~\citep{poole1985spatial, clinton2004statistical}, we construct a one-dimensional latent preference embedding for interest groups based on their bill positions. By aggregating LLM and GNN annotations along with the MapLight dataset, we generate latent interest scores using an item response theory (IRT) model to provide a unified measure of their positions. To estimate these scores, we apply the graded model~\citep{samejima1968estimation} within the mirt (Multidimensional Item Response Theory) package~\citep{chalmers2012mirt} in R, which allows us to handle ordered categorical labels. We focus on \textit{Support} and \textit{Oppose} labels, excluding \textit{\updated{Engage}} to maintain consistency with established approaches in political analysis and to better capture distinct policy preferences. To ensure reliable estimation, we retain only interest groups that have lobbied on at least 10 bills and bills that have been lobbied by at least 10 different groups. After this filtering, we derive latent preferences for 1,796 interest groups and 2,020 bills. \todo{[reliability score]}


\paragraph{Comparison of Interest Group Preferences: CFscores vs. Bill Position-Based Estimates}
Campaign finance scores (CFscores), provided by DIME~\citep{bonica2023database}, are widely used to represent interest groups' ideological positions based on campaign finance data. To compare these with our bill position-based latent preferences—reflecting a more direct measure of lobbying activity—we examine 218 interest groups with identical names in both datasets.
Since CFscores are reported for individual Congresses, we first compute each group's mean CFscore across all Congresses and compare it to their bill position-based latent preference. The Pearson correlation~\footnote{\url{https://docs.scipy.org/doc/scipy/reference/generated/scipy.stats.pearsonr.html}} between the two is 0.191, suggesting a weak but positive relationship. This indicates that while campaign contributions and lobbying activities may be related, they capture distinct aspects of interest group behavior.

% Interest groups are organizations that pursue specific interests, and their preferences are likely to remain consistent even as Congress changes. To verify whether our data reflects the consistent interests of these groups, we compare the interest group scores across different Congresses, in contrast with the CFscores. Both datasets are normalized using z-score normalization, setting the mean to 0 and the variance to 1. We then compare the within-variance and between-variance of the interest group scores. A lower within-variance indicates that the group's score remains consistent across Congresses, suggesting stable interests, while a higher between-variance indicates better differentiation of latent preferences among the groups. The within-variance for the DIME score is 0.784, while ours is 0.745, and the between-variance values are 0.216 and 0.255, respectively. These results suggest that our data better captures the stable and distinguishable latent preferences of the interest groups.







==> sup_table/fractional_qoi.tex <==
\begin{table*}
\centering
\caption{Fractional Logistic Regression Results: Effect of Firm Size on Predicted Probability of Lobbying Position}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lccccc}
% \toprule
 & No Fixed Effects & Year FE & Year + NAICS FE & Year FE + Log PPENT + Log COGS & Year + NAICS FE + Log PPENT + Log COGS \\
\midrule
Support & -0.055 (0.032)$^*$ & -0.052 (0.031)$^*$ & -0.060 (0.035)$^*$ & -0.028 (0.057) & -0.092 (0.067)$^*$ \\
Oppose  & -0.011 (0.012)   & -0.009 (0.011)   & -0.013 (0.012)   & -0.001 (0.014) & 0.005 (0.020) \\
Amend   & -0.015 (0.017)   & -0.009 (0.017)   &  0.020 (0.017)   & -0.136 (0.044)$^{***}$ & -0.007 (0.037) \\
Monitor &  0.082 (0.043)$^*$ &  0.070 (0.041)$^*$ &  0.056 (0.041)   &  0.140 (0.073)$^*$ &  0.088 (0.078) \\
\midrule
\multicolumn{6}{l}{\footnotesize Note: Clustered standard errors are in parentheses. *p$<$0.1; **p$<$0.05; ***p$<$0.01.}
\end{tabular}%
}
\label{tab:SI_fractional_qoi}
\end{table*}



==> table/gnn_prediction_score.tex <==
\begin{table}[]
\centering
\caption{GNN Prediction}
\label{tab:gnn_prediction}
\begin{tabular}{cc|ccc}
% \toprule
Accuracy                  & F1                        & \begin{tabular}[c]{@{}c@{}}F1\\ Support\end{tabular} & \begin{tabular}[c]{@{}c@{}}F1\\ Oppose\end{tabular} & \begin{tabular}[c]{@{}c@{}}F1\\ Amend\&Monitor\end{tabular} \\ \midrule
\multicolumn{1}{r}{80.29 \tiny{\textpm 0.19}} & \multicolumn{1}{r}{77.08 \tiny{\textpm0.30}} & \multicolumn{1}{|r}{84.59 \tiny{\textpm0.24}} & \multicolumn{1}{r}{70.80 \tiny{\textpm0.68}} & \multicolumn{1}{r}{75.84 \tiny{\textpm0.17}} \\ \bottomrule
\end{tabular}
\end{table}

==> table/llm_bill_position_example.tex <==
\begin{table*}[]
\centering
\renewcommand{\arraystretch}{1.5} % 행의 높이를 1.5배로 설정
% \begin{tabular}{@{}c p{5cm}p{7.5cm} c@{}} % Bill Id 열을 중앙 정렬로 수정
\caption{Bill Position Example Annotated by LLM}
\begin{tabular}{@{}c p{5cm}p{7.5cm} p{1.5cm}@{}} % Bill Id 열을 중앙 정렬로 수정
\toprule
Bill Id  & \multicolumn{1}{c}{Bill Title}                                                         & \multicolumn{1}{c}{Lobbying Description}                                                                          & Bill Position \\ \midrule
H.R.1421 & Improving Access to Medicare Coverage Act of 2017                                      & S. 568, \colorbox{supportcolor}{\textbf{H.R. 1421}}, Improving Access to Medicare Coverage Act - Discussed our \colorbox{supportcolor}{support for/endorsed bill.}           & \colorbox{supportcolor}{\textbf{Support}}       \\ \cline{1-4}
H.R.1249 & Leahy-Smith America Invents Act & \colorbox{opposecolor}{defeat S. 23 and \textbf{H.R. 1249}}, and pass funding only bill for USPTO                                                             & \colorbox{opposecolor}{\textbf{Oppose}}        \\ \cline{1-4}
H.R.9    & Innovation Act                                                                         & \colorbox{amendcolor}{Advocacy for changes to \textbf{H.R. 9}}, the Innovation Act regarding the potential impact of provisions on the ability... & \colorbox{lightgray}{\textbf{Others}} (\colorbox{amendcolor}{Amend})         \\ \cline{1-4}
S.744    & Border Security, Economic Opportunity, and Immigration Modernization Act               & ... \colorbox{monitorcolor}{Legislation watched includes: S 169, \textbf{S 744}}, HR 2131, HR 459, HR 15 and S 600.                                 & \colorbox{lightgray}{\textbf{Others}} (\colorbox{monitorcolor}{Monitor})       \\ \bottomrule
\end{tabular}
\end{table*}




% \begin{table*}[]
% \begin{tabular}{@{}cclp{6cm}@{}} % p{6cm}로 Lobbying Description 열의 너비를 6cm로 설정
% \toprule
% Bill Position & Bill Id  & \multicolumn{1}{c}{Bill Title}                                                                                                   & \multicolumn{1}{c}{Lobbying Description}                                                                          \\ \midrule
% Support       & H.R.1421 & Improving Access to Medicare Coverage Act of 2017                                                                                & S. 568, H.R. 1421, Improving Access to Medicare Coverage Act - Discussed our support for/endorsed bill.           \\ \cline{1-4}
% Oppose        & H.R.1754 & \begin{tabular}[c]{@{}l@{}}Department of State, Foreign Operations, and Related\\ Programs Appropriations Act, 2016\end{tabular} & Against H.R. 1754, Horseracing Integrity Act of 2019.                                                             \\ \cline{1-4}
% Amend         & H.R.9    & Innovation Act                                                                                                                   & Advocacy for changes to H.R. 9, the Innovation Act regarding the potential impact of provisions on the ability... \\ \cline{1-4}
% Monitor       & S.744    & \begin{tabular}[c]{@{}l@{}}Border Security, Economic Opportunity, and Immigration \\ Modernization Act\end{tabular}              & ... Legislation watched includes: S 169, S 744, HR 2131, HR 459, HR 15 and S 600.                                 \\ \bottomrule
% \end{tabular}
% \caption{Example table with uniform column width}
% \end{table*}



